FlowInOne:Unifying Multimodal Generation as Image-in, Image-out Flow Matching

Multimodal generation has long been dominated by text-driven pipelines where language dictates vision but cannot reason or create within it. We challenge this paradigm by asking whether all modalities, including textual descriptions, spatial layouts, and editing instructions, can be unified into a single visual representation. We present FlowInOne, a framework that reformulates multimodal generation as a purely visual flow, converting all inputs into visual prompts and enabling a clean image-in, image-out pipeline governed by a single flow matching model. This vision-centric formulation naturally eliminates cross-modal alignment bottlenecks, noise scheduling, and task-specific architectural branches, unifying text-to-image generation, layout-guided editing, and visual instruction following under one coherent paradigm. To support this, we introduce VisPrompt-5M, a large-scale dataset of 5 million visual prompt pairs spanning diverse tasks including physics-aware force dynamics and trajectory prediction, alongside VP-Bench, a rigorously curated benchmark assessing instruction faithfulness, spatial precision, visual realism, and content consistency. Extensive experiments demonstrate that FlowInOne achieves state-of-the-art performance among open-source models across all unified generation tasks while remaining competitive with leading commercial systems, thereby establishing a new foundation for fully vision-centric generative modeling, in which perception and creation coexist within a unified continuous visual space. Our code and models are released on https://csu-jpg.github.io/FlowInOne.github.io/

==> Figures/tex/generation_prompts.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{Figures/figure/generation_prompts.pdf}
    \caption{Unified Meta-Instruction for Fair Evaluation.}
    % \vspace{-6mm}
    \label{fig:gen_prompts}
\end{figure*}

==> Figures/tex/teaser.tex <==
\twocolumn
[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    % \vspace{-6mm}
    \captionsetup{type=figure}
\includegraphics[width=\linewidth]{Figures/figure/teaser.pdf}
    % \vspace{-10mm}
    \captionof{figure}{\textbf{We propose \modelname, a general and simple framework that directly evolves one modality to another using \FM with no additional conditioning}.
    This is enabled using a vanilla transformer without cross-attention, achieving comparable performance with \sota models on (a) \ttoi generation, and (b) various other tasks, without requiring task specific architectures. 
    }
    \label{fig:teaser}
\end{center}%
}]
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{Figures/figure/teaser.pdf}
%   \caption{\textbf{We propose \modelname, a general and simple framework that directly evolves one modality to another using \FM with no additional conditioning.}
%   \label{fig:teaser}
% \end{figure*}


==> Tables/configuration.tex <==
\begin{table}[htbp]
\centering
\small
\scalebox{1}{
\begin{tabular}{l|ccccc}
model & depth & width & mlp & heads & \#params \\ \hline
\modelname-B & 12 & 768 & 3072 & 12 & 153M \\
\modelname-XL & 28 & 1152 & 4608 & 16 & 698M \\
\modelname-H & 36 & 1280 & 5120 & 20 & 1.1B 
\end{tabular}
}
\caption{
\textbf{Architecture Configuration of \modelname.}
Following prior work, we scale up DiT blocks across three configurations.
}
\label{tab:flowtok_configuration}
\end{table}

==> Tables/quan_eval_human.tex <==
\begin{table}[htbp]
  \centering
  \vspace{-8mm}
  \caption{Evaluation On visual instruction benchmark by professional engineers assessing the generation success rates. }
  \label{tab:human-eval}
  \begin{tabular}{l|cccccccc|c}
    \toprule
    \textbf{Method} & \textbf{C2I} & \textbf{T2I} & \textbf{TIE} & \textbf{FU} & \textbf{TBE} & \textbf{TU} & \textbf{VME} & \textbf{DE} & \textbf{All} \\
    \midrule
    Nano Banana & .602 & .804 & .271 & .250 & .300 & .000 & .229 & .792 & .406 \\
    Omnigen2 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 \\
    Kontext & .000 & .000 & .043 & .000 & .000 & .000 & .000 & .100 & .018 \\
    Qwen-IE-2509 & .067 & .000 & .029 & .000 & .000 & .000 & .000 & .000 & .012 \\
    \midrule
    \textbf{FlowInOne (Ours)} & \textbf{.800} & \textbf{.695} & \textbf{.257} & \textbf{.705} & \textbf{.200} & \textbf{.280} & \textbf{.255} & \textbf{.400} & \textbf{.449} \\
    \bottomrule
  \end{tabular}
  \label{tab:quan-human}
  \vspace{-8mm}
\end{table}
%修改总表

==> sec/3_preliminary.tex <==
\section{Preliminaries}
\paragraph{Image-to-image generation.}
In the conventional sense, image-to-image (I2I) refers to learning a mapping from a given input image to another domain or attribute. 
Typical tasks include paired or unpaired cross-domain translation~\cite{xiao2025thermalgen,Nobis2025FractionalDB,Liu2023I2SBIS,liu2023flow,zhou2024denoising}, as well as various forms of image restoration and reconstruction~\cite{wang2025residualdiffusionbridgemodel,liu2025latentharmonysynergisticunified}. Representative approaches are primarily based on adversarial frameworks such as conditional GANs\cite{mirza2014conditionalgenerativeadversarialnets} and CycleGAN\cite{zhu2020unpairedimagetoimagetranslationusing}, or, under diffusion priors, perform editing and synthesis via noise injection and denoising~\cite{meng2022sdeditguidedimagesynthesis}. 
These methods often rely on task-specific control channels and interfaces to encode geometric or semantic constraints.
In contrast, we render heterogeneous instructions—text, bounding boxes, arrows, doodles, trajectories etc.—into a unified visual instruction, thereby converging multiple forms of control into a single image input.
Within a shared latent space, we then employ Flow Matching to learn the continuous transport from the visual instruction state to the target image state. 
This unified paradigm simultaneously covers text-to-image generation (with text prompt rendered as an image) and a variety of image editing tasks, without requiring per-task conditional branches or noise schedules.
Formally, denote latent of the input image as $Z_{\mathrm{TI}}\in\mathbb{R}^{H\times W\times C}$ and the latent of the target image as $Z_{\mathrm{I}}\in\mathbb{R}^{H\times W\times C}$. Then, in the shared representation, this paradigm learn the time dependent velocity field \( v_{\theta} \) to drive the deterministic evolution.
\begin{equation}\label{eq1}
\frac{dZ_t}{dt}=v_\theta(Z_t,t),\quad Z_{t=0}=Z_{\mathrm{TI}},\quad Z_{t=1}=Z_{\mathrm{I}}
\end{equation}
where $t\in[0,1]$ denotes the time parameter of the continuous transport. This process, without introducing noise schedules or multi-branch conditioning, realizes an end-to-end mapping and a unified solution from visual instructions image to the target image.
\paragraph{Flow Matching.}
This method\cite{lipman2023flowmatchinggenerativemodeling,liu2022flowstraightfastlearning,liu2024instaflowstephighqualitydiffusionbased} formulates generative modeling as a continuous transport from a source distribution $p_0$ to a target distribution $p_1$ over the interval $[0,1]$. It learns a time-dependent velocity field that drives latent variables along an ordinary differential equation in~\ref{eq1}.
During training, a differentiable bridging path is constructed between sample pairs $(z_0,z_1)$:
\begin{equation} \label{eq2}
z_t=t\left.z_1+\left(1-(1-\sigma_{\min})t\right)z_0,\right.
\end{equation}
which yields the ground-truth velocity at each time step for supervision:
\begin{equation} \label{eq3}
v_t^\star=\frac{\partial z_t}{\partial t}= z_1-(1-\sigma_{\min})z_0
\end{equation}
The model approximates $v_\theta(z_t,t) $ along this path by minimizing the MSE between the predicted velocity field and the true velocity. 
At inference, the target latent is obtained by integrating the learned field over time, solving the ODE from a given initial state up to $t=1$.
Unlike diffusion~\cite{ddpm,song2021ddim}, FM does not rely on noise scheduling, and the source distribution need not be Gaussian—only isomorphic to the target. 
In this work, the source distribution is non-Gaussian: we obtain the posterior $z_0$ from a unified visual input via a visual encoder and a Variational Autoencoder(VAE), and the target latent $z_1$ via image VAE encoding.
Both latents are isomorphic within a shared space, in which we learn the continuous transport from the visual instruction state to the image state.

==> sec/bk.tex <==
%%abs

Traditional text-to-image (T2I) and text-image-to-image (TI2I) generation methods are built upon heterogeneous modeling paradigms, which hampers the establishment of a common latent space for bidirectional alignment and consistent reasoning.
In this paper, we introduce \modelname, a framework that unifies T2I and TI2I tasks under a cohesive image-to-image (I2I) paradigm. 
\modelname transforms textual descriptions into visual elements and incorporates them, alongside visual markers and the input image, as purely visual modalities.
Within this unified visual space, the method performs flow matching to promote generation consistency.
\modelname employs a visual encoder to extract representations that integrate semantic and geometric information, modeling the continuous trajectory from a mixed text–image state to a purely visual state within a homogeneous domain. 
By encoding the target image as a compact one-dimensional (1D) token sequence, \modelname enables position-aware flow matching within a shared sequence space. This design obviates Gaussian denoising and complex conditioning mechanisms, while alleviating the structural mismatch between 1D sequences and 2D latent spaces. 
Compared with conventional 2D latent representations, the proposed 1D tokenization substantially reduces redundancy and computational overhead, yielding more efficient sampling.
Moreover, a homogeneous sequence structure together with positional encodings enhances semantic coherence and spatial alignment.
Extensive experiments show that \modelname delivers substantial gains in zero-shot generation and precise image editing, and exhibits strong scalability across diverse instruction types and multilingual scenarios.

%% introduction
Bridging different modalities is essential for comprehending the diverse forms of data that represent our world, encompassing both understanding and generation.
In multimodal understanding, extensive research has focused on designing architectures that project different modalities into a shared latent space~\cite{li2019visualbert,lu2019vilbert,radford2021learning,jia2021scaling,cho2021unifying,wang2021simvlm,li2022blip,jaegle2021perceiver,alayrac2022flamingo,driess2023palm}. These approaches have significantly advanced cross-modal representation learning and real-world understanding by leveraging a common latent space between modalities.

In contrast, multimodal generation (\eg, text-to-image generation) follows a different paradigm, primarily relying on the diffusion process~\cite{sohl2015deep,song2019generative,ho2020denoising,peebles2023scalable,liu2024alleviating}, where the source modality (\eg, text) serves as a conditioning signal to guide the denoising process.
Various conditioning mechanisms have been explored, including concatenation~\cite{bao2023all}, cross-attention~\cite{rombach2022high,chen2024pixartalpha}, conditioning embeddings~\cite{peebles2023scalable}, and hybrid strategies~\cite{esser2024scaling,kim2025democratizing}. While effective, these approaches introduce substantial complexity, requiring intricate conditioning mechanisms and noise scheduling.
This naturally raises an important question:
\textit{Can we unify multimodal understanding and generation by enabling direct transitions within a shared latent space?}

To address this question, we revisit flow matching~\cite{lipmanflow,albergo2022building,liuflow}—a modern generative framework that learns a direct path from noise to data, enabling faster convergence and accelerated sampling, leading to state-of-the-art multimodal generation results~\cite{esser2024scaling,flux2024}.
Unlike diffusion models, flow matching is not constrained to using noise as the source distribution; instead, it only requires the source and target distributions to share the same shape. Pioneering works~\cite{albergo2022building,liu2023i2sbimagetoimageschrodingerbridge,shi2023diffusion,tong2023simulation,zhou2023denoising} have demonstrated its effectiveness in learning direct mappings within the same modality (\eg, image-to-image generation).
Meanwhile, CrossFlow~\cite{liu2024flowing} extends flow matching to cross-modal learning by mapping text into a 2D latent space to match the shape of image embeddings, paving the way for new possibilities.
However, while this approach simplifies the overall pipeline, it still operates on 2D latent representations.

As a result, the additional computational overhead introduced by the text variational autoencoder~\cite{kingma2013auto} in CrossFlow makes it slower than modern text-to-image diffusion models like SD1.5 and SD2.1~\cite{rombach2022high}, ultimately contradicting its original goal of efficiency.

To this end, we introduce \modelname, a minimal framework that enables seamless \textbf{Flow}ing of \textbf{Tok}ens across text and image—the two most prevalent modalities.
At the core of \modelname, both text and images are encoded into compact 1D latent tokens within a unified space, enabling direct flow matching between them. On the text side, \modelname employs a pre-trained text encoder~\cite{radford2021learning} to extract initial 1D text embeddings. Since these embeddings typically reside in a higher-dimensional space than image latents, \modelname introduces a lightweight text projector to map text embeddings into a low-dimensional variational latent space.
% , regularized by a KL-divergence loss to ensure a smooth distribution for sampling. 
% To maintain semantic integrity, we enforce a contrastive feature alignment objective, ensuring that the projected text tokens remain well-aligned with an additional learned embedding via MLPs.
On the image side, \modelname builds on recent advancements in image tokenization~\cite{yu2024image,kim2025democratizing} to encode images into compact 1D latent tokens. Specifically, we enhance \tokenizername~\cite{kim2025democratizing} by integrating RoPE~\cite{su2021roformer} and SwiGLU FFN~\cite{shazeer2020glu}, improving positional information handling and reconstruction quality. To enable direct flow matching, we align the number of image latent tokens $K$ in \tokenizername to match the text encoder’s output sequence length ($K=77$ for CLIP text encoder).

By integrating these simple yet effective designs across text and image modalities, \modelname represents both in the same 1D low-dimensional space with shape $77 \times 16$ (77 tokens, each with 16 dimensions). This compact representation is 3.3$\times$ smaller than typical 2D flow matching shapes~\cite{sdvae} of $32 \times 32 \times 4$ for image resolutions of 256. This alignment enables fast, direct flow matching and seamless evolution between the two modalities.

Unlike standard flow matching models~\cite{ma2024sit,lipmanflow,liuflow}, \modelname eliminates the need for intricate conditioning mechanisms, offering a fully self-attention-based generative model. This allows for direct flow across modalities without additional complexity. Unlike CrossFlow~\cite{liu2024flowing}, which converts text into 2D embeddings, \modelname retains the 1D structure of text embeddings, avoiding the need for flattening and transformation into 2D. This simplifies the framework while eliminating reliance on heavy parametric contrastive losses for semantic preservation.


As a result, \modelname offers a streamlined and resource-efficient training process. Its largest variant, \modelname-H (1.1B), supports a batch size of 8K on 8 A100 GPUs without requiring gradient checkpointing or gradient accumulation. In contrast, recent text-to-image models of similar scale typically require 32 to 64 A100 GPUs to train with a batch size of only 2K~\cite{rombach2022high,chen2024pixartalpha}. Moreover, \modelname converges significantly faster, as shown in, with \modelname-H completing training in just 26.1 8-A100 days—far less than SD 2.1~\cite{rombach2022high}, which requires 1041.6 8-A100 GPU days.

Inference is also highly efficient, with \modelname achieving over 10$\times$ the throughput of Show-o~\cite{xie2024show} and CrossFlow~\cite{liu2024flowing}, as shown in. This dramatically reduces computational costs, making text-to-image research far more accessible. To ensure full reproducibility, we train \modelname exclusively on publicly available datasets, avoiding reliance on high-quality proprietary data. Remarkably, despite its minimalist design and reduced data requirements, \modelname achieves state-of-the-art text-to-image performance.

Beyond text-to-image generation, \modelname seamlessly extends to image-to-text generation, maintaining strong performance under the same minimalist framework. We believe our work establishes a strong foundation for future research in generalized cross-modality generation. To support further advancements, all code will be released.

